Invariant tori for multi-dimensional integrable hamiltonians coupled to a single thermostat

This paper demonstrates sufficient conditions for the existence of KAM tori in a singly thermostated, integrable hamiltonian system with $n$ degrees of freedom with a focus on the generalized, variable-mass thermostats of order 2--which include the Nos\'e thermostat, the logistic thermostat of Tapias, Bravetti and Sanders, and the Winkler thermostat. It extends Theorem 3.2 of Legoll, Luskin & Moeckel, (Non-ergodicity of Nos\'e-Hoover dynamics, Nonlinearity, 22 (2009), pp. 1673--1694) to prove that a "typical" singly thermostated, integrable, real-analytic hamiltonian possesses a positive-measure set of invariant tori when the thermostat is weakly coupled. It also demonstrates a class of integrable hamiltonians, which, for a full-measure set of couplings, satisfies the same conclusion.

==> nhnd/nhnd-3d-60-30-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1144,1209){\makebox(0,0){\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(1792,1086){\makebox(0,0){\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(2440,963){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(3088,840){\makebox(0,0){\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(3735,717){\makebox(0,0){\strut{}1}}%
      \csname LTb\endcsname%%
      \put(4221,742){\makebox(0,0)[l]{\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(4475,887){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(4730,1032){\makebox(0,0)[l]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(4984,1177){\makebox(0,0)[l]{\strut{}1}}%
      \csname LTb\endcsname%%
      \put(5239,1321){\makebox(0,0)[l]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(5493,1466){\makebox(0,0)[l]{\strut{}2}}%
      \csname LTb\endcsname%%
      \put(5748,1611){\makebox(0,0)[l]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(821,2022){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(821,2182){\makebox(0,0)[r]{\strut{}-1.5}}%
      \csname LTb\endcsname%%
      \put(821,2342){\makebox(0,0)[r]{\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(821,2503){\makebox(0,0)[r]{\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(821,2662){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(821,2822){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(821,2983){\makebox(0,0)[r]{\strut{}1}}%
      \csname LTb\endcsname%%
      \put(821,3143){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(821,3303){\makebox(0,0)[r]{\strut{}2}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2010,750){\makebox(0,0){\strut{}$x$}}%
      \csname LTb\endcsname%%
      \put(5781,1083){\makebox(0,0){\strut{}$s-s_o$ ($× 10^{-2}$)}}%
      \csname LTb\endcsname%%
      \put(199,2662){\rotatebox{-270}{\makebox(0,0){\strut{}$S$ ($× 10^{-3}$)}}}%
      \csname LTb\endcsname%%
      \put(3390,4681){\makebox(0,0){\strut{}$a=19$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-2}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-60-30-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-60-30-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1144,1209){\makebox(0,0){\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(1792,1086){\makebox(0,0){\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(2440,963){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(3088,840){\makebox(0,0){\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(3735,717){\makebox(0,0){\strut{}1}}%
      \csname LTb\endcsname%%
      \put(4221,742){\makebox(0,0)[l]{\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(4475,887){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(4730,1031){\makebox(0,0)[l]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(4984,1176){\makebox(0,0)[l]{\strut{}1}}%
      \csname LTb\endcsname%%
      \put(5239,1321){\makebox(0,0)[l]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(5493,1466){\makebox(0,0)[l]{\strut{}2}}%
      \csname LTb\endcsname%%
      \put(5748,1611){\makebox(0,0)[l]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(821,2021){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(821,2182){\makebox(0,0)[r]{\strut{}-1.5}}%
      \csname LTb\endcsname%%
      \put(821,2342){\makebox(0,0)[r]{\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(821,2503){\makebox(0,0)[r]{\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(821,2662){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(821,2822){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(821,2983){\makebox(0,0)[r]{\strut{}1}}%
      \csname LTb\endcsname%%
      \put(821,3143){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(821,3304){\makebox(0,0)[r]{\strut{}2}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2010,750){\makebox(0,0){\strut{}$x$}}%
      \csname LTb\endcsname%%
      \put(5781,1083){\makebox(0,0){\strut{}$s-s_o$ ($× 10^{-2}$)}}%
      \csname LTb\endcsname%%
      \put(199,2662){\rotatebox{-270}{\makebox(0,0){\strut{}$S$ ($× 10^{-3}$)}}}%
      \csname LTb\endcsname%%
      \put(3390,4681){\makebox(0,0){\strut{}$a=19$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-2}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-60-30-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-60-30-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1133,1211){\makebox(0,0){\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(1787,1087){\makebox(0,0){\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(2440,963){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(3094,839){\makebox(0,0){\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(3746,715){\makebox(0,0){\strut{}1}}%
      \csname LTb\endcsname%%
      \put(4188,723){\makebox(0,0)[l]{\strut{}-1.8}}%
      \csname LTb\endcsname%%
      \put(4380,833){\makebox(0,0)[l]{\strut{}-1.6}}%
      \csname LTb\endcsname%%
      \put(4572,942){\makebox(0,0)[l]{\strut{}-1.4}}%
      \csname LTb\endcsname%%
      \put(4764,1051){\makebox(0,0)[l]{\strut{}-1.2}}%
      \csname LTb\endcsname%%
      \put(4957,1161){\makebox(0,0)[l]{\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(5149,1270){\makebox(0,0)[l]{\strut{}-0.8}}%
      \csname LTb\endcsname%%
      \put(5341,1379){\makebox(0,0)[l]{\strut{}-0.6}}%
      \csname LTb\endcsname%%
      \put(5533,1489){\makebox(0,0)[l]{\strut{}-0.4}}%
      \csname LTb\endcsname%%
      \put(5725,1598){\makebox(0,0)[l]{\strut{}-0.2}}%
      \csname LTb\endcsname%%
      \put(5917,1708){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(821,2029){\makebox(0,0)[r]{\strut{}-8}}%
      \csname LTb\endcsname%%
      \put(821,2187){\makebox(0,0)[r]{\strut{}-6}}%
      \csname LTb\endcsname%%
      \put(821,2346){\makebox(0,0)[r]{\strut{}-4}}%
      \csname LTb\endcsname%%
      \put(821,2504){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(821,2662){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(821,2820){\makebox(0,0)[r]{\strut{}2}}%
      \csname LTb\endcsname%%
      \put(821,2979){\makebox(0,0)[r]{\strut{}4}}%
      \csname LTb\endcsname%%
      \put(821,3137){\makebox(0,0)[r]{\strut{}6}}%
      \csname LTb\endcsname%%
      \put(821,3296){\makebox(0,0)[r]{\strut{}8}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2010,750){\makebox(0,0){\strut{}$x$}}%
      \csname LTb\endcsname%%
      \put(5781,1083){\makebox(0,0){\strut{}$s-s_o$ ($× 10^{-6}$)}}%
      \csname LTb\endcsname%%
      \put(199,2662){\rotatebox{-270}{\makebox(0,0){\strut{}$S$ ($× 10^{-7}$)}}}%
      \csname LTb\endcsname%%
      \put(3390,4681){\makebox(0,0){\strut{}$a=1$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-6}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-60-30-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-60-30-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1133,1211){\makebox(0,0){\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(1787,1087){\makebox(0,0){\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(2440,963){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(3094,839){\makebox(0,0){\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(3746,715){\makebox(0,0){\strut{}1}}%
      \csname LTb\endcsname%%
      \put(4188,723){\makebox(0,0)[l]{\strut{}-1.8}}%
      \csname LTb\endcsname%%
      \put(4380,833){\makebox(0,0)[l]{\strut{}-1.6}}%
      \csname LTb\endcsname%%
      \put(4572,942){\makebox(0,0)[l]{\strut{}-1.4}}%
      \csname LTb\endcsname%%
      \put(4764,1051){\makebox(0,0)[l]{\strut{}-1.2}}%
      \csname LTb\endcsname%%
      \put(4957,1161){\makebox(0,0)[l]{\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(5149,1270){\makebox(0,0)[l]{\strut{}-0.8}}%
      \csname LTb\endcsname%%
      \put(5341,1379){\makebox(0,0)[l]{\strut{}-0.6}}%
      \csname LTb\endcsname%%
      \put(5533,1489){\makebox(0,0)[l]{\strut{}-0.4}}%
      \csname LTb\endcsname%%
      \put(5725,1598){\makebox(0,0)[l]{\strut{}-0.2}}%
      \csname LTb\endcsname%%
      \put(5917,1708){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(821,2029){\makebox(0,0)[r]{\strut{}-8}}%
      \csname LTb\endcsname%%
      \put(821,2187){\makebox(0,0)[r]{\strut{}-6}}%
      \csname LTb\endcsname%%
      \put(821,2346){\makebox(0,0)[r]{\strut{}-4}}%
      \csname LTb\endcsname%%
      \put(821,2504){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(821,2662){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(821,2820){\makebox(0,0)[r]{\strut{}2}}%
      \csname LTb\endcsname%%
      \put(821,2979){\makebox(0,0)[r]{\strut{}4}}%
      \csname LTb\endcsname%%
      \put(821,3137){\makebox(0,0)[r]{\strut{}6}}%
      \csname LTb\endcsname%%
      \put(821,3296){\makebox(0,0)[r]{\strut{}8}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2010,750){\makebox(0,0){\strut{}$x$}}%
      \csname LTb\endcsname%%
      \put(5781,1083){\makebox(0,0){\strut{}$s-s_o$ ($× 10^{-6}$)}}%
      \csname LTb\endcsname%%
      \put(199,2662){\rotatebox{-270}{\makebox(0,0){\strut{}$S$ ($× 10^{-7}$)}}}%
      \csname LTb\endcsname%%
      \put(3390,4681){\makebox(0,0){\strut{}$a=1$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-6}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-60-30-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-90-90-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1762,1161){\makebox(0,0){\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(2270,1161){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(2779,1161){\makebox(0,0){\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(3288,1161){\makebox(0,0){\strut{}1}}%
      \csname LTb\endcsname%%
      \put(3796,1161){\makebox(0,0){\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(4305,1161){\makebox(0,0){\strut{}2}}%
      \csname LTb\endcsname%%
      \put(4814,1161){\makebox(0,0){\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(1466,2186){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(1466,2371){\makebox(0,0)[r]{\strut{}-1.5}}%
      \csname LTb\endcsname%%
      \put(1466,2555){\makebox(0,0)[r]{\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(1466,2741){\makebox(0,0)[r]{\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(1466,2926){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1466,3111){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(1466,3296){\makebox(0,0)[r]{\strut{}1}}%
      \csname LTb\endcsname%%
      \put(1466,3481){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(1466,3666){\makebox(0,0)[r]{\strut{}2}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3390,506){\makebox(0,0){\strut{}$s-s_o$ ($× 10^{-2}$)}}%
      \csname LTb\endcsname%%
      \put(844,2926){\rotatebox{-270}{\makebox(0,0){\strut{}$S$ ($× 10^{-3}$)}}}%
      \csname LTb\endcsname%%
      \put(3390,4681){\makebox(0,0){\strut{}$a=19$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-2}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-90-90-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-90-90-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1761,1161){\makebox(0,0){\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(2270,1161){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(2779,1161){\makebox(0,0){\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(3288,1161){\makebox(0,0){\strut{}1}}%
      \csname LTb\endcsname%%
      \put(3796,1161){\makebox(0,0){\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(4305,1161){\makebox(0,0){\strut{}2}}%
      \csname LTb\endcsname%%
      \put(4814,1161){\makebox(0,0){\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(1466,2186){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(1466,2371){\makebox(0,0)[r]{\strut{}-1.5}}%
      \csname LTb\endcsname%%
      \put(1466,2555){\makebox(0,0)[r]{\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(1466,2741){\makebox(0,0)[r]{\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(1466,2926){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1466,3111){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(1466,3296){\makebox(0,0)[r]{\strut{}1}}%
      \csname LTb\endcsname%%
      \put(1466,3482){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(1466,3667){\makebox(0,0)[r]{\strut{}2}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3390,506){\makebox(0,0){\strut{}$s-s_o$ ($× 10^{-2}$)}}%
      \csname LTb\endcsname%%
      \put(844,2926){\rotatebox{-270}{\makebox(0,0){\strut{}$S$ ($× 10^{-3}$)}}}%
      \csname LTb\endcsname%%
      \put(3390,4681){\makebox(0,0){\strut{}$a=19$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-2}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-90-90-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-90-90-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1696,1161){\makebox(0,0){\strut{}-1.8}}%
      \csname LTb\endcsname%%
      \put(2080,1161){\makebox(0,0){\strut{}-1.6}}%
      \csname LTb\endcsname%%
      \put(2464,1161){\makebox(0,0){\strut{}-1.4}}%
      \csname LTb\endcsname%%
      \put(2848,1161){\makebox(0,0){\strut{}-1.2}}%
      \csname LTb\endcsname%%
      \put(3233,1161){\makebox(0,0){\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(3616,1161){\makebox(0,0){\strut{}-0.8}}%
      \csname LTb\endcsname%%
      \put(4000,1161){\makebox(0,0){\strut{}-0.6}}%
      \csname LTb\endcsname%%
      \put(4384,1161){\makebox(0,0){\strut{}-0.4}}%
      \csname LTb\endcsname%%
      \put(4768,1161){\makebox(0,0){\strut{}-0.2}}%
      \csname LTb\endcsname%%
      \put(5152,1161){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1466,2195){\makebox(0,0)[r]{\strut{}-8}}%
      \csname LTb\endcsname%%
      \put(1466,2378){\makebox(0,0)[r]{\strut{}-6}}%
      \csname LTb\endcsname%%
      \put(1466,2560){\makebox(0,0)[r]{\strut{}-4}}%
      \csname LTb\endcsname%%
      \put(1466,2743){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(1466,2926){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1466,3109){\makebox(0,0)[r]{\strut{}2}}%
      \csname LTb\endcsname%%
      \put(1466,3292){\makebox(0,0)[r]{\strut{}4}}%
      \csname LTb\endcsname%%
      \put(1466,3475){\makebox(0,0)[r]{\strut{}6}}%
      \csname LTb\endcsname%%
      \put(1466,3658){\makebox(0,0)[r]{\strut{}8}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3390,506){\makebox(0,0){\strut{}$s-s_o$ ($× 10^{-6}$)}}%
      \csname LTb\endcsname%%
      \put(844,2926){\rotatebox{-270}{\makebox(0,0){\strut{}$S$ ($× 10^{-7}$)}}}%
      \csname LTb\endcsname%%
      \put(3390,4681){\makebox(0,0){\strut{}$a=1$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-6}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-90-90-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-90-90-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1696,1161){\makebox(0,0){\strut{}-1.8}}%
      \csname LTb\endcsname%%
      \put(2080,1161){\makebox(0,0){\strut{}-1.6}}%
      \csname LTb\endcsname%%
      \put(2464,1161){\makebox(0,0){\strut{}-1.4}}%
      \csname LTb\endcsname%%
      \put(2848,1161){\makebox(0,0){\strut{}-1.2}}%
      \csname LTb\endcsname%%
      \put(3233,1161){\makebox(0,0){\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(3616,1161){\makebox(0,0){\strut{}-0.8}}%
      \csname LTb\endcsname%%
      \put(4000,1161){\makebox(0,0){\strut{}-0.6}}%
      \csname LTb\endcsname%%
      \put(4384,1161){\makebox(0,0){\strut{}-0.4}}%
      \csname LTb\endcsname%%
      \put(4768,1161){\makebox(0,0){\strut{}-0.2}}%
      \csname LTb\endcsname%%
      \put(5152,1161){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1466,2195){\makebox(0,0)[r]{\strut{}-8}}%
      \csname LTb\endcsname%%
      \put(1466,2378){\makebox(0,0)[r]{\strut{}-6}}%
      \csname LTb\endcsname%%
      \put(1466,2560){\makebox(0,0)[r]{\strut{}-4}}%
      \csname LTb\endcsname%%
      \put(1466,2743){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(1466,2926){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1466,3109){\makebox(0,0)[r]{\strut{}2}}%
      \csname LTb\endcsname%%
      \put(1466,3292){\makebox(0,0)[r]{\strut{}4}}%
      \csname LTb\endcsname%%
      \put(1466,3475){\makebox(0,0)[r]{\strut{}6}}%
      \csname LTb\endcsname%%
      \put(1466,3658){\makebox(0,0)[r]{\strut{}8}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3390,506){\makebox(0,0){\strut{}$s-s_o$ ($× 10^{-6}$)}}%
      \csname LTb\endcsname%%
      \put(844,2926){\rotatebox{-270}{\makebox(0,0){\strut{}$S$ ($× 10^{-7}$)}}}%
      \csname LTb\endcsname%%
      \put(3390,4681){\makebox(0,0){\strut{}$a=1$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-6}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-90-90-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-delta-H-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(596,839){\makebox(0,0)[r]{\strut{}-6}}%
      \csname LTb\endcsname%%
      \put(596,1382){\makebox(0,0)[r]{\strut{}-5}}%
      \csname LTb\endcsname%%
      \put(596,1926){\makebox(0,0)[r]{\strut{}-4}}%
      \csname LTb\endcsname%%
      \put(596,2469){\makebox(0,0)[r]{\strut{}-3}}%
      \csname LTb\endcsname%%
      \put(596,3012){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(596,3555){\makebox(0,0)[r]{\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(596,4098){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(708,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1395,448){\makebox(0,0){\strut{}2000}}%
      \csname LTb\endcsname%%
      \put(2083,448){\makebox(0,0){\strut{}4000}}%
      \csname LTb\endcsname%%
      \put(2771,448){\makebox(0,0){\strut{}6000}}%
      \csname LTb\endcsname%%
      \put(3458,448){\makebox(0,0){\strut{}8000}}%
      \csname LTb\endcsname%%
      \put(4146,448){\makebox(0,0){\strut{}10000}}%
      \csname LTb\endcsname%%
      \put(4833,448){\makebox(0,0){\strut{}12000}}%
      \csname LTb\endcsname%%
      \put(5521,448){\makebox(0,0){\strut{}14000}}%
      \csname LTb\endcsname%%
      \put(6209,448){\makebox(0,0){\strut{}16000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}$Δ 𝐇$ ($× 10^{-8}$)}}}%
      \csname LTb\endcsname%%
      \put(6392,2559){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3524,142){\makebox(0,0){\strut{}step}}%
      \csname LTb\endcsname%%
      \put(3524,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3524,4773){\makebox(0,0){\strut{}$a=19$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-2}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-delta-H-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-delta-H-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(596,840){\makebox(0,0)[r]{\strut{}-6}}%
      \csname LTb\endcsname%%
      \put(596,1383){\makebox(0,0)[r]{\strut{}-5}}%
      \csname LTb\endcsname%%
      \put(596,1926){\makebox(0,0)[r]{\strut{}-4}}%
      \csname LTb\endcsname%%
      \put(596,2469){\makebox(0,0)[r]{\strut{}-3}}%
      \csname LTb\endcsname%%
      \put(596,3012){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(596,3555){\makebox(0,0)[r]{\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(596,4098){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(708,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1395,448){\makebox(0,0){\strut{}2000}}%
      \csname LTb\endcsname%%
      \put(2083,448){\makebox(0,0){\strut{}4000}}%
      \csname LTb\endcsname%%
      \put(2771,448){\makebox(0,0){\strut{}6000}}%
      \csname LTb\endcsname%%
      \put(3458,448){\makebox(0,0){\strut{}8000}}%
      \csname LTb\endcsname%%
      \put(4146,448){\makebox(0,0){\strut{}10000}}%
      \csname LTb\endcsname%%
      \put(4833,448){\makebox(0,0){\strut{}12000}}%
      \csname LTb\endcsname%%
      \put(5521,448){\makebox(0,0){\strut{}14000}}%
      \csname LTb\endcsname%%
      \put(6209,448){\makebox(0,0){\strut{}16000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}$Δ 𝐇$ ($× 10^{-8}$)}}}%
      \csname LTb\endcsname%%
      \put(6392,2559){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3524,142){\makebox(0,0){\strut{}step}}%
      \csname LTb\endcsname%%
      \put(3524,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3524,4773){\makebox(0,0){\strut{}$a=19$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-2}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-delta-H-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-delta-H-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(820,972){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(820,1408){\makebox(0,0)[r]{\strut{}-1.5}}%
      \csname LTb\endcsname%%
      \put(820,1844){\makebox(0,0)[r]{\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(820,2280){\makebox(0,0)[r]{\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(820,2716){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(820,3152){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(820,3588){\makebox(0,0)[r]{\strut{}1}}%
      \csname LTb\endcsname%%
      \put(820,4024){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(820,4460){\makebox(0,0)[r]{\strut{}2}}%
      \csname LTb\endcsname%%
      \put(932,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1592,448){\makebox(0,0){\strut{}2000}}%
      \csname LTb\endcsname%%
      \put(2252,448){\makebox(0,0){\strut{}4000}}%
      \csname LTb\endcsname%%
      \put(2913,448){\makebox(0,0){\strut{}6000}}%
      \csname LTb\endcsname%%
      \put(3573,448){\makebox(0,0){\strut{}8000}}%
      \csname LTb\endcsname%%
      \put(4233,448){\makebox(0,0){\strut{}10000}}%
      \csname LTb\endcsname%%
      \put(4893,448){\makebox(0,0){\strut{}12000}}%
      \csname LTb\endcsname%%
      \put(5554,448){\makebox(0,0){\strut{}14000}}%
      \csname LTb\endcsname%%
      \put(6214,448){\makebox(0,0){\strut{}16000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}$Δ 𝐇$ ($× 10^{-12}$)}}}%
      \csname LTb\endcsname%%
      \put(6392,2559){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3636,142){\makebox(0,0){\strut{}step}}%
      \csname LTb\endcsname%%
      \put(3636,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3636,4773){\makebox(0,0){\strut{}$a=1$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-6}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-delta-H-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-delta-H-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(820,972){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(820,1408){\makebox(0,0)[r]{\strut{}-1.5}}%
      \csname LTb\endcsname%%
      \put(820,1844){\makebox(0,0)[r]{\strut{}-1}}%
      \csname LTb\endcsname%%
      \put(820,2280){\makebox(0,0)[r]{\strut{}-0.5}}%
      \csname LTb\endcsname%%
      \put(820,2716){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(820,3152){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(820,3588){\makebox(0,0)[r]{\strut{}1}}%
      \csname LTb\endcsname%%
      \put(820,4024){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(820,4460){\makebox(0,0)[r]{\strut{}2}}%
      \csname LTb\endcsname%%
      \put(932,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1592,448){\makebox(0,0){\strut{}2000}}%
      \csname LTb\endcsname%%
      \put(2252,448){\makebox(0,0){\strut{}4000}}%
      \csname LTb\endcsname%%
      \put(2913,448){\makebox(0,0){\strut{}6000}}%
      \csname LTb\endcsname%%
      \put(3573,448){\makebox(0,0){\strut{}8000}}%
      \csname LTb\endcsname%%
      \put(4233,448){\makebox(0,0){\strut{}10000}}%
      \csname LTb\endcsname%%
      \put(4893,448){\makebox(0,0){\strut{}12000}}%
      \csname LTb\endcsname%%
      \put(5554,448){\makebox(0,0){\strut{}14000}}%
      \csname LTb\endcsname%%
      \put(6214,448){\makebox(0,0){\strut{}16000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}$Δ 𝐇$ ($× 10^{-12}$)}}}%
      \csname LTb\endcsname%%
      \put(6392,2559){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3636,142){\makebox(0,0){\strut{}step}}%
      \csname LTb\endcsname%%
      \put(3636,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3636,4773){\makebox(0,0){\strut{}$a=1$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-6}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-delta-H-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-delta-ptheta-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,743){\makebox(0,0)[r]{\strut{}-16}}%
      \csname LTb\endcsname%%
      \put(708,1168){\makebox(0,0)[r]{\strut{}-14}}%
      \csname LTb\endcsname%%
      \put(708,1592){\makebox(0,0)[r]{\strut{}-12}}%
      \csname LTb\endcsname%%
      \put(708,2016){\makebox(0,0)[r]{\strut{}-10}}%
      \csname LTb\endcsname%%
      \put(708,2440){\makebox(0,0)[r]{\strut{}-8}}%
      \csname LTb\endcsname%%
      \put(708,2865){\makebox(0,0)[r]{\strut{}-6}}%
      \csname LTb\endcsname%%
      \put(708,3289){\makebox(0,0)[r]{\strut{}-4}}%
      \csname LTb\endcsname%%
      \put(708,3713){\makebox(0,0)[r]{\strut{}-2}}%
      \csname LTb\endcsname%%
      \put(708,4137){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(820,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1494,448){\makebox(0,0){\strut{}2000}}%
      \csname LTb\endcsname%%
      \put(2168,448){\makebox(0,0){\strut{}4000}}%
      \csname LTb\endcsname%%
      \put(2842,448){\makebox(0,0){\strut{}6000}}%
      \csname LTb\endcsname%%
      \put(3515,448){\makebox(0,0){\strut{}8000}}%
      \csname LTb\endcsname%%
      \put(4189,448){\makebox(0,0){\strut{}10000}}%
      \csname LTb\endcsname%%
      \put(4863,448){\makebox(0,0){\strut{}12000}}%
      \csname LTb\endcsname%%
      \put(5537,448){\makebox(0,0){\strut{}14000}}%
      \csname LTb\endcsname%%
      \put(6211,448){\makebox(0,0){\strut{}16000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}$Δ p_{θ}$ ($× 10^{-15}$)}}}%
      \csname LTb\endcsname%%
      \put(6392,2559){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3580,142){\makebox(0,0){\strut{}step}}%
      \csname LTb\endcsname%%
      \put(3580,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3580,4773){\makebox(0,0){\strut{}$a=19$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-2}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-delta-ptheta-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-delta-ptheta-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(596,826){\makebox(0,0)[r]{\strut{}-5}}%
      \csname LTb\endcsname%%
      \put(596,1350){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(596,1874){\makebox(0,0)[r]{\strut{}5}}%
      \csname LTb\endcsname%%
      \put(596,2398){\makebox(0,0)[r]{\strut{}10}}%
      \csname LTb\endcsname%%
      \put(596,2921){\makebox(0,0)[r]{\strut{}15}}%
      \csname LTb\endcsname%%
      \put(596,3445){\makebox(0,0)[r]{\strut{}20}}%
      \csname LTb\endcsname%%
      \put(596,3969){\makebox(0,0)[r]{\strut{}25}}%
      \csname LTb\endcsname%%
      \put(708,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1395,448){\makebox(0,0){\strut{}2000}}%
      \csname LTb\endcsname%%
      \put(2083,448){\makebox(0,0){\strut{}4000}}%
      \csname LTb\endcsname%%
      \put(2771,448){\makebox(0,0){\strut{}6000}}%
      \csname LTb\endcsname%%
      \put(3458,448){\makebox(0,0){\strut{}8000}}%
      \csname LTb\endcsname%%
      \put(4146,448){\makebox(0,0){\strut{}10000}}%
      \csname LTb\endcsname%%
      \put(4833,448){\makebox(0,0){\strut{}12000}}%
      \csname LTb\endcsname%%
      \put(5521,448){\makebox(0,0){\strut{}14000}}%
      \csname LTb\endcsname%%
      \put(6209,448){\makebox(0,0){\strut{}16000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}$Δ p_{θ}$ ($× 10^{-15}$)}}}%
      \csname LTb\endcsname%%
      \put(6392,2559){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3524,142){\makebox(0,0){\strut{}step}}%
      \csname LTb\endcsname%%
      \put(3524,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3524,4773){\makebox(0,0){\strut{}$a=19$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-2}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-delta-ptheta-a19_0-T0_5-logdelta-2-stepsize0_0625-time1024_0-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-delta-ptheta-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,1342){\makebox(0,0)[r]{\strut{}-15}}%
      \csname LTb\endcsname%%
      \put(708,2184){\makebox(0,0)[r]{\strut{}-10}}%
      \csname LTb\endcsname%%
      \put(708,3026){\makebox(0,0)[r]{\strut{}-5}}%
      \csname LTb\endcsname%%
      \put(708,3869){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(820,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1494,448){\makebox(0,0){\strut{}2000}}%
      \csname LTb\endcsname%%
      \put(2168,448){\makebox(0,0){\strut{}4000}}%
      \csname LTb\endcsname%%
      \put(2842,448){\makebox(0,0){\strut{}6000}}%
      \csname LTb\endcsname%%
      \put(3515,448){\makebox(0,0){\strut{}8000}}%
      \csname LTb\endcsname%%
      \put(4189,448){\makebox(0,0){\strut{}10000}}%
      \csname LTb\endcsname%%
      \put(4863,448){\makebox(0,0){\strut{}12000}}%
      \csname LTb\endcsname%%
      \put(5537,448){\makebox(0,0){\strut{}14000}}%
      \csname LTb\endcsname%%
      \put(6211,448){\makebox(0,0){\strut{}16000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}$Δ p_{θ}$ ($× 10^{-15}$)}}}%
      \csname LTb\endcsname%%
      \put(6392,2559){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3580,142){\makebox(0,0){\strut{}step}}%
      \csname LTb\endcsname%%
      \put(3580,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3580,4773){\makebox(0,0){\strut{}$a=1$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-6}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-delta-ptheta-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-3d-delta-ptheta-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,1342){\makebox(0,0)[r]{\strut{}-15}}%
      \csname LTb\endcsname%%
      \put(708,2184){\makebox(0,0)[r]{\strut{}-10}}%
      \csname LTb\endcsname%%
      \put(708,3026){\makebox(0,0)[r]{\strut{}-5}}%
      \csname LTb\endcsname%%
      \put(708,3869){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(820,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(1494,448){\makebox(0,0){\strut{}2000}}%
      \csname LTb\endcsname%%
      \put(2168,448){\makebox(0,0){\strut{}4000}}%
      \csname LTb\endcsname%%
      \put(2842,448){\makebox(0,0){\strut{}6000}}%
      \csname LTb\endcsname%%
      \put(3515,448){\makebox(0,0){\strut{}8000}}%
      \csname LTb\endcsname%%
      \put(4189,448){\makebox(0,0){\strut{}10000}}%
      \csname LTb\endcsname%%
      \put(4863,448){\makebox(0,0){\strut{}12000}}%
      \csname LTb\endcsname%%
      \put(5537,448){\makebox(0,0){\strut{}14000}}%
      \csname LTb\endcsname%%
      \put(6211,448){\makebox(0,0){\strut{}16000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}$Δ p_{θ}$ ($× 10^{-15}$)}}}%
      \csname LTb\endcsname%%
      \put(6392,2559){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3580,142){\makebox(0,0){\strut{}step}}%
      \csname LTb\endcsname%%
      \put(3580,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3580,4773){\makebox(0,0){\strut{}$a=1$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-6}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-3d-delta-ptheta-a1_0-T0_5-logdelta-6-stepsize0_0625-time1024_0-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-ratio-llm-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(708,1420){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,2188){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,2955){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,3723){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,4491){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(1316,448){\makebox(0,0){\strut{}$-1$}}%
      \csname LTb\endcsname%%
      \put(2033,448){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(2751,448){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(3469,448){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(4187,448){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4904,448){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5622,448){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6340,448){\makebox(0,0){\strut{}$6$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$ω_1/ω_2$}}}%
      \csname LTb\endcsname%%
      \put(6392,2763){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3580,142){\makebox(0,0){\strut{}$\ln T$}}%
      \csname LTb\endcsname%%
      \put(3580,4875){\makebox(0,0){\strut{}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2249,2572){\makebox(0,0){\strut{}$a=0.7$}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2376,2188){\makebox(0,0){\strut{}$a=0.4$}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2808,1804){\makebox(0,0){\strut{}$a=0.1$}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(1944,2955){\makebox(0,0){\strut{}$a=1.0$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-ratio-llm-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-ratios-1024-a1-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,651){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(708,1377){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,2102){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,2827){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,3553){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,4278){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(1765,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(2715,448){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(3665,448){\makebox(0,0){\strut{}600}}%
      \csname LTb\endcsname%%
      \put(4615,448){\makebox(0,0){\strut{}800}}%
      \csname LTb\endcsname%%
      \put(5565,448){\makebox(0,0){\strut{}1000}}%
      \csname LTb\endcsname%%
      \put(5791,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5791,1371){\makebox(0,0)[l]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(5791,2090){\makebox(0,0)[l]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(5791,2810){\makebox(0,0)[l]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(5791,3529){\makebox(0,0)[l]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(5791,4248){\makebox(0,0)[l]{\strut{}0.5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude}}}%
      \csname LTb\endcsname%%
      \put(6341,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude ($× 10^{-2}$)}}}%
      \csname LTb\endcsname%%
      \put(3249,142){\makebox(0,0){\strut{}$k$ (frequency number)}}%
      \csname LTb\endcsname%%
      \put(3249,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3249,4773){\makebox(0,0){\strut{}$a=1$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-2}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-ratios-1024-a1-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-ratios-1024-a1-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,651){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(708,1377){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,2102){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,2827){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,3553){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,4278){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(1765,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(2715,448){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(3665,448){\makebox(0,0){\strut{}600}}%
      \csname LTb\endcsname%%
      \put(4615,448){\makebox(0,0){\strut{}800}}%
      \csname LTb\endcsname%%
      \put(5565,448){\makebox(0,0){\strut{}1000}}%
      \csname LTb\endcsname%%
      \put(5791,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5791,1370){\makebox(0,0)[l]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(5791,2088){\makebox(0,0)[l]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(5791,2806){\makebox(0,0)[l]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(5791,3524){\makebox(0,0)[l]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(5791,4242){\makebox(0,0)[l]{\strut{}0.5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude}}}%
      \csname LTb\endcsname%%
      \put(6341,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude ($× 10^{-2}$)}}}%
      \csname LTb\endcsname%%
      \put(3249,142){\makebox(0,0){\strut{}$k$ (frequency number)}}%
      \csname LTb\endcsname%%
      \put(3249,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3249,4773){\makebox(0,0){\strut{}$a=1$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-2}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-ratios-1024-a1-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-ratios-1024-a19-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,651){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(708,1376){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,2102){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,2827){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,3552){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,4277){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(1765,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(2715,448){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(3665,448){\makebox(0,0){\strut{}600}}%
      \csname LTb\endcsname%%
      \put(4615,448){\makebox(0,0){\strut{}800}}%
      \csname LTb\endcsname%%
      \put(5565,448){\makebox(0,0){\strut{}1000}}%
      \csname LTb\endcsname%%
      \put(5791,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5791,1284){\makebox(0,0)[l]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(5791,1916){\makebox(0,0)[l]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(5791,2548){\makebox(0,0)[l]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(5791,3180){\makebox(0,0)[l]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(5791,3811){\makebox(0,0)[l]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(5791,4443){\makebox(0,0)[l]{\strut{}0.6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude}}}%
      \csname LTb\endcsname%%
      \put(6341,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude ($× 10^{-2}$)}}}%
      \csname LTb\endcsname%%
      \put(3249,142){\makebox(0,0){\strut{}$k$ (frequency number)}}%
      \csname LTb\endcsname%%
      \put(3249,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3249,4773){\makebox(0,0){\strut{}$a=19$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-2}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-ratios-1024-a19-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-ratios-1024-a19-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,651){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(708,1376){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,2102){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,2827){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,3552){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,4277){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(1765,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(2715,448){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(3665,448){\makebox(0,0){\strut{}600}}%
      \csname LTb\endcsname%%
      \put(4615,448){\makebox(0,0){\strut{}800}}%
      \csname LTb\endcsname%%
      \put(5565,448){\makebox(0,0){\strut{}1000}}%
      \csname LTb\endcsname%%
      \put(5791,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5791,1282){\makebox(0,0)[l]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(5791,1912){\makebox(0,0)[l]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(5791,2541){\makebox(0,0)[l]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(5791,3171){\makebox(0,0)[l]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(5791,3801){\makebox(0,0)[l]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(5791,4431){\makebox(0,0)[l]{\strut{}0.6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude}}}%
      \csname LTb\endcsname%%
      \put(6341,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude ($× 10^{-2}$)}}}%
      \csname LTb\endcsname%%
      \put(3249,142){\makebox(0,0){\strut{}$k$ (frequency number)}}%
      \csname LTb\endcsname%%
      \put(3249,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3249,4773){\makebox(0,0){\strut{}$a=19$, $T=1/2$, $h=1/16$, $B=1024$, $δ=10^{-2}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-ratios-1024-a19-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-ratios-a1-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(820,649){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(820,1061){\makebox(0,0)[r]{\strut{}0.05}}%
      \csname LTb\endcsname%%
      \put(820,1474){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(820,1886){\makebox(0,0)[r]{\strut{}0.15}}%
      \csname LTb\endcsname%%
      \put(820,2299){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(820,2711){\makebox(0,0)[r]{\strut{}0.25}}%
      \csname LTb\endcsname%%
      \put(820,3123){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(820,3536){\makebox(0,0)[r]{\strut{}0.35}}%
      \csname LTb\endcsname%%
      \put(820,3948){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(820,4361){\makebox(0,0)[r]{\strut{}0.45}}%
      \csname LTb\endcsname%%
      \put(1823,448){\makebox(0,0){\strut{}50}}%
      \csname LTb\endcsname%%
      \put(2731,448){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(3640,448){\makebox(0,0){\strut{}150}}%
      \csname LTb\endcsname%%
      \put(4549,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(5458,448){\makebox(0,0){\strut{}250}}%
      \csname LTb\endcsname%%
      \put(5679,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5679,1349){\makebox(0,0)[l]{\strut{}0.05}}%
      \csname LTb\endcsname%%
      \put(5679,2045){\makebox(0,0)[l]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(5679,2742){\makebox(0,0)[l]{\strut{}0.15}}%
      \csname LTb\endcsname%%
      \put(5679,3438){\makebox(0,0)[l]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(5679,4135){\makebox(0,0)[l]{\strut{}0.25}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude}}}%
      \csname LTb\endcsname%%
      \put(6341,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude ($× 10^{-6}$)}}}%
      \csname LTb\endcsname%%
      \put(3249,142){\makebox(0,0){\strut{}$k$ (frequency number)}}%
      \csname LTb\endcsname%%
      \put(3249,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3249,4773){\makebox(0,0){\strut{}$a=1$, $T=1/2$, $h=1/16$, $B=256$, $δ=10^{-6}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-ratios-a1-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-ratios-a1-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(820,649){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(820,1061){\makebox(0,0)[r]{\strut{}0.05}}%
      \csname LTb\endcsname%%
      \put(820,1474){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(820,1886){\makebox(0,0)[r]{\strut{}0.15}}%
      \csname LTb\endcsname%%
      \put(820,2299){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(820,2711){\makebox(0,0)[r]{\strut{}0.25}}%
      \csname LTb\endcsname%%
      \put(820,3123){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(820,3536){\makebox(0,0)[r]{\strut{}0.35}}%
      \csname LTb\endcsname%%
      \put(820,3948){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(820,4361){\makebox(0,0)[r]{\strut{}0.45}}%
      \csname LTb\endcsname%%
      \put(1823,448){\makebox(0,0){\strut{}50}}%
      \csname LTb\endcsname%%
      \put(2731,448){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(3640,448){\makebox(0,0){\strut{}150}}%
      \csname LTb\endcsname%%
      \put(4549,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(5458,448){\makebox(0,0){\strut{}250}}%
      \csname LTb\endcsname%%
      \put(5679,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5679,1349){\makebox(0,0)[l]{\strut{}0.05}}%
      \csname LTb\endcsname%%
      \put(5679,2045){\makebox(0,0)[l]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(5679,2742){\makebox(0,0)[l]{\strut{}0.15}}%
      \csname LTb\endcsname%%
      \put(5679,3438){\makebox(0,0)[l]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(5679,4135){\makebox(0,0)[l]{\strut{}0.25}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude}}}%
      \csname LTb\endcsname%%
      \put(6341,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude ($× 10^{-6}$)}}}%
      \csname LTb\endcsname%%
      \put(3249,142){\makebox(0,0){\strut{}$k$ (frequency number)}}%
      \csname LTb\endcsname%%
      \put(3249,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3249,4773){\makebox(0,0){\strut{}$a=1$, $T=1/2$, $h=1/16$, $B=256$, $δ=10^{-6}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-ratios-a1-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-ratios-a19-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(820,649){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(820,1061){\makebox(0,0)[r]{\strut{}0.05}}%
      \csname LTb\endcsname%%
      \put(820,1474){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(820,1886){\makebox(0,0)[r]{\strut{}0.15}}%
      \csname LTb\endcsname%%
      \put(820,2299){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(820,2711){\makebox(0,0)[r]{\strut{}0.25}}%
      \csname LTb\endcsname%%
      \put(820,3123){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(820,3536){\makebox(0,0)[r]{\strut{}0.35}}%
      \csname LTb\endcsname%%
      \put(820,3948){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(820,4361){\makebox(0,0)[r]{\strut{}0.45}}%
      \csname LTb\endcsname%%
      \put(1844,448){\makebox(0,0){\strut{}50}}%
      \csname LTb\endcsname%%
      \put(2775,448){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(3706,448){\makebox(0,0){\strut{}150}}%
      \csname LTb\endcsname%%
      \put(4637,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(5567,448){\makebox(0,0){\strut{}250}}%
      \csname LTb\endcsname%%
      \put(5791,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5791,1338){\makebox(0,0)[l]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(5791,2025){\makebox(0,0)[l]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(5791,2711){\makebox(0,0)[l]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(5791,3397){\makebox(0,0)[l]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(5791,4083){\makebox(0,0)[l]{\strut{}0.5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude}}}%
      \csname LTb\endcsname%%
      \put(6341,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude ($× 10^{-6}$)}}}%
      \csname LTb\endcsname%%
      \put(3305,142){\makebox(0,0){\strut{}$k$ (frequency number)}}%
      \csname LTb\endcsname%%
      \put(3305,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3305,4773){\makebox(0,0){\strut{}$a=19$, $T=1/2$, $h=1/16$, $B=256$, $δ=10^{-6}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-ratios-a19-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-ratios-a19-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(820,649){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(820,1061){\makebox(0,0)[r]{\strut{}0.05}}%
      \csname LTb\endcsname%%
      \put(820,1474){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(820,1886){\makebox(0,0)[r]{\strut{}0.15}}%
      \csname LTb\endcsname%%
      \put(820,2299){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(820,2711){\makebox(0,0)[r]{\strut{}0.25}}%
      \csname LTb\endcsname%%
      \put(820,3123){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(820,3536){\makebox(0,0)[r]{\strut{}0.35}}%
      \csname LTb\endcsname%%
      \put(820,3948){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(820,4361){\makebox(0,0)[r]{\strut{}0.45}}%
      \csname LTb\endcsname%%
      \put(1844,448){\makebox(0,0){\strut{}50}}%
      \csname LTb\endcsname%%
      \put(2775,448){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(3706,448){\makebox(0,0){\strut{}150}}%
      \csname LTb\endcsname%%
      \put(4637,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(5567,448){\makebox(0,0){\strut{}250}}%
      \csname LTb\endcsname%%
      \put(5791,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5791,1338){\makebox(0,0)[l]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(5791,2025){\makebox(0,0)[l]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(5791,2711){\makebox(0,0)[l]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(5791,3397){\makebox(0,0)[l]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(5791,4083){\makebox(0,0)[l]{\strut{}0.5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude}}}%
      \csname LTb\endcsname%%
      \put(6341,2559){\rotatebox{-270}{\makebox(0,0){\strut{}amplitude ($× 10^{-6}$)}}}%
      \csname LTb\endcsname%%
      \put(3305,142){\makebox(0,0){\strut{}$k$ (frequency number)}}%
      \csname LTb\endcsname%%
      \put(3305,4467){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3305,4773){\makebox(0,0){\strut{}$a=19$, $T=1/2$, $h=1/16$, $B=256$, $δ=10^{-6}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-ratios-a19-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-resp-1024-eps0_01-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,1255){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,1859){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,2462){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,3065){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(708,3668){\makebox(0,0)[r]{\strut{}0.6}}%
      \csname LTb\endcsname%%
      \put(708,4272){\makebox(0,0)[r]{\strut{}0.7}}%
      \csname LTb\endcsname%%
      \put(708,4875){\makebox(0,0)[r]{\strut{}0.8}}%
      \csname LTb\endcsname%%
      \put(820,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(2193,448){\makebox(0,0){\strut{}5}}%
      \csname LTb\endcsname%%
      \put(3567,448){\makebox(0,0){\strut{}10}}%
      \csname LTb\endcsname%%
      \put(4940,448){\makebox(0,0){\strut{}15}}%
      \csname LTb\endcsname%%
      \put(6314,448){\makebox(0,0){\strut{}20}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$ω_1/ω_2$}}}%
      \csname LTb\endcsname%%
      \put(6392,2763){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3580,142){\makebox(0,0){\strut{}$a$}}%
      \csname LTb\endcsname%%
      \put(3580,4875){\makebox(0,0){\strut{}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3567,2462){\makebox(0,0){\strut{}$T=1/2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-resp-1024-eps0_01-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-resp-1024-eps0_01-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,1255){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,1859){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,2462){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,3065){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(708,3668){\makebox(0,0)[r]{\strut{}0.6}}%
      \csname LTb\endcsname%%
      \put(708,4272){\makebox(0,0)[r]{\strut{}0.7}}%
      \csname LTb\endcsname%%
      \put(708,4875){\makebox(0,0)[r]{\strut{}0.8}}%
      \csname LTb\endcsname%%
      \put(820,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(2193,448){\makebox(0,0){\strut{}5}}%
      \csname LTb\endcsname%%
      \put(3567,448){\makebox(0,0){\strut{}10}}%
      \csname LTb\endcsname%%
      \put(4940,448){\makebox(0,0){\strut{}15}}%
      \csname LTb\endcsname%%
      \put(6314,448){\makebox(0,0){\strut{}20}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$ω_1/ω_2$}}}%
      \csname LTb\endcsname%%
      \put(6392,2763){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3580,142){\makebox(0,0){\strut{}$a$}}%
      \csname LTb\endcsname%%
      \put(3580,4875){\makebox(0,0){\strut{}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3567,2462){\makebox(0,0){\strut{}$T=1/2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-resp-1024-eps0_01-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-resp-1024-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,1255){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,1859){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,2462){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,3065){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(708,3668){\makebox(0,0)[r]{\strut{}0.6}}%
      \csname LTb\endcsname%%
      \put(708,4272){\makebox(0,0)[r]{\strut{}0.7}}%
      \csname LTb\endcsname%%
      \put(708,4875){\makebox(0,0)[r]{\strut{}0.8}}%
      \csname LTb\endcsname%%
      \put(820,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(2193,448){\makebox(0,0){\strut{}5}}%
      \csname LTb\endcsname%%
      \put(3567,448){\makebox(0,0){\strut{}10}}%
      \csname LTb\endcsname%%
      \put(4940,448){\makebox(0,0){\strut{}15}}%
      \csname LTb\endcsname%%
      \put(6314,448){\makebox(0,0){\strut{}20}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$ω_1/ω_2$}}}%
      \csname LTb\endcsname%%
      \put(6392,2763){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3580,142){\makebox(0,0){\strut{}$a$}}%
      \csname LTb\endcsname%%
      \put(3580,4875){\makebox(0,0){\strut{}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3567,2462){\makebox(0,0){\strut{}$T=1/2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-resp-1024-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-resp-1024-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,1255){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,1859){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,2462){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,3065){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(708,3668){\makebox(0,0)[r]{\strut{}0.6}}%
      \csname LTb\endcsname%%
      \put(708,4272){\makebox(0,0)[r]{\strut{}0.7}}%
      \csname LTb\endcsname%%
      \put(708,4875){\makebox(0,0)[r]{\strut{}0.8}}%
      \csname LTb\endcsname%%
      \put(820,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(2193,448){\makebox(0,0){\strut{}5}}%
      \csname LTb\endcsname%%
      \put(3567,448){\makebox(0,0){\strut{}10}}%
      \csname LTb\endcsname%%
      \put(4940,448){\makebox(0,0){\strut{}15}}%
      \csname LTb\endcsname%%
      \put(6314,448){\makebox(0,0){\strut{}20}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$ω_1/ω_2$}}}%
      \csname LTb\endcsname%%
      \put(6392,2763){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3580,142){\makebox(0,0){\strut{}$a$}}%
      \csname LTb\endcsname%%
      \put(3580,4875){\makebox(0,0){\strut{}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3567,2462){\makebox(0,0){\strut{}$T=1/2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-resp-1024-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-resp-256-eps0_01-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,1255){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,1859){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,2462){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,3065){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(708,3668){\makebox(0,0)[r]{\strut{}0.6}}%
      \csname LTb\endcsname%%
      \put(708,4272){\makebox(0,0)[r]{\strut{}0.7}}%
      \csname LTb\endcsname%%
      \put(708,4875){\makebox(0,0)[r]{\strut{}0.8}}%
      \csname LTb\endcsname%%
      \put(820,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(2193,448){\makebox(0,0){\strut{}5}}%
      \csname LTb\endcsname%%
      \put(3567,448){\makebox(0,0){\strut{}10}}%
      \csname LTb\endcsname%%
      \put(4940,448){\makebox(0,0){\strut{}15}}%
      \csname LTb\endcsname%%
      \put(6314,448){\makebox(0,0){\strut{}20}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$ω_1/ω_2$}}}%
      \csname LTb\endcsname%%
      \put(6392,2763){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3580,142){\makebox(0,0){\strut{}$a$}}%
      \csname LTb\endcsname%%
      \put(3580,4875){\makebox(0,0){\strut{}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3567,2462){\makebox(0,0){\strut{}$T=1/2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-resp-256-eps0_01-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-resp-256-eps0_01-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,1255){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,1859){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,2462){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,3065){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(708,3668){\makebox(0,0)[r]{\strut{}0.6}}%
      \csname LTb\endcsname%%
      \put(708,4272){\makebox(0,0)[r]{\strut{}0.7}}%
      \csname LTb\endcsname%%
      \put(708,4875){\makebox(0,0)[r]{\strut{}0.8}}%
      \csname LTb\endcsname%%
      \put(820,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(2193,448){\makebox(0,0){\strut{}5}}%
      \csname LTb\endcsname%%
      \put(3567,448){\makebox(0,0){\strut{}10}}%
      \csname LTb\endcsname%%
      \put(4940,448){\makebox(0,0){\strut{}15}}%
      \csname LTb\endcsname%%
      \put(6314,448){\makebox(0,0){\strut{}20}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$ω_1/ω_2$}}}%
      \csname LTb\endcsname%%
      \put(6392,2763){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3580,142){\makebox(0,0){\strut{}$a$}}%
      \csname LTb\endcsname%%
      \put(3580,4875){\makebox(0,0){\strut{}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3567,2462){\makebox(0,0){\strut{}$T=1/2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-resp-256-eps0_01-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-resp-256-logistic-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,1255){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,1859){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,2462){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,3065){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(708,3668){\makebox(0,0)[r]{\strut{}0.6}}%
      \csname LTb\endcsname%%
      \put(708,4272){\makebox(0,0)[r]{\strut{}0.7}}%
      \csname LTb\endcsname%%
      \put(708,4875){\makebox(0,0)[r]{\strut{}0.8}}%
      \csname LTb\endcsname%%
      \put(820,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(2193,448){\makebox(0,0){\strut{}5}}%
      \csname LTb\endcsname%%
      \put(3567,448){\makebox(0,0){\strut{}10}}%
      \csname LTb\endcsname%%
      \put(4940,448){\makebox(0,0){\strut{}15}}%
      \csname LTb\endcsname%%
      \put(6314,448){\makebox(0,0){\strut{}20}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$ω_1/ω_2$}}}%
      \csname LTb\endcsname%%
      \put(6392,2763){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3580,142){\makebox(0,0){\strut{}$a$}}%
      \csname LTb\endcsname%%
      \put(3580,4875){\makebox(0,0){\strut{}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3567,2462){\makebox(0,0){\strut{}$T=1/2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-resp-256-logistic-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-freq-resp-256-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,1255){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,1859){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,2462){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,3065){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(708,3668){\makebox(0,0)[r]{\strut{}0.6}}%
      \csname LTb\endcsname%%
      \put(708,4272){\makebox(0,0)[r]{\strut{}0.7}}%
      \csname LTb\endcsname%%
      \put(708,4875){\makebox(0,0)[r]{\strut{}0.8}}%
      \csname LTb\endcsname%%
      \put(820,448){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(2193,448){\makebox(0,0){\strut{}5}}%
      \csname LTb\endcsname%%
      \put(3567,448){\makebox(0,0){\strut{}10}}%
      \csname LTb\endcsname%%
      \put(4940,448){\makebox(0,0){\strut{}15}}%
      \csname LTb\endcsname%%
      \put(6314,448){\makebox(0,0){\strut{}20}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$ω_1/ω_2$}}}%
      \csname LTb\endcsname%%
      \put(6392,2763){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3580,142){\makebox(0,0){\strut{}$a$}}%
      \csname LTb\endcsname%%
      \put(3580,4875){\makebox(0,0){\strut{}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3567,2462){\makebox(0,0){\strut{}$T=1/2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-freq-resp-256-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-nose-freq-rat-a=1e-1-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\relax
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(820,1056){\makebox(0,0)[r]{\strut{}0.25}}%
      \csname LTb\endcsname%%
      \put(820,1706){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(820,2355){\makebox(0,0)[r]{\strut{}0.35}}%
      \csname LTb\endcsname%%
      \put(820,3005){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(820,3654){\makebox(0,0)[r]{\strut{}0.45}}%
      \csname LTb\endcsname%%
      \put(820,4304){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(1473,448){\makebox(0,0){\strut{}1}}%
      \csname LTb\endcsname%%
      \put(2555,448){\makebox(0,0){\strut{}2}}%
      \csname LTb\endcsname%%
      \put(3637,448){\makebox(0,0){\strut{}3}}%
      \csname LTb\endcsname%%
      \put(4718,448){\makebox(0,0){\strut{}4}}%
      \csname LTb\endcsname%%
      \put(5800,448){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}normal/internal frequency}}}%
      \csname LTb\endcsname%%
      \put(6392,2763){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3636,142){\makebox(0,0){\strut{}$ λ $ (homogeneity degree)}}%
      \csname LTb\endcsname%%
      \put(3636,4875){\makebox(0,0){\strut{}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(5800,3054){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=10, η=10$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(5199,2570){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=10, η=8$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(5172,3425){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=8, η=10$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4718,2098){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=8, η=8$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4448,1883){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=10, η=6$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4421,2794){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=6, η=10$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4100,1583){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=8, η=6$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4073,2518){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=6, η=8$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3637,3456){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=6, η=6$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3482,3326){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=10, η=4$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3455,4258){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=4, η=10$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3276,3163){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=8, η=4$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3249,4094){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=4, η=8$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2987,2963){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=6, η=4$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2960,3893){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=4, η=6$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2555,2667){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=4, η=4$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2194,2334){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=10, η=2$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2167,3338){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=2, η=10$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2122,2327){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=8, η=2$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2095,3332){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=2, η=8$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2014,2294){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=6, η=2$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(1987,3302){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=2, η=6$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(1834,2325){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=4, η=2$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(1806,3255){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=2, η=4$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(1473,2617){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=2, η=2$}}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-nose-freq-rat-a=1e-1-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-nose-freq-rat-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\relax
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(820,1095){\makebox(0,0)[r]{\strut{}0.08}}%
      \csname LTb\endcsname%%
      \put(820,1916){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(820,2738){\makebox(0,0)[r]{\strut{}0.12}}%
      \csname LTb\endcsname%%
      \put(820,3560){\makebox(0,0)[r]{\strut{}0.14}}%
      \csname LTb\endcsname%%
      \put(820,4381){\makebox(0,0)[r]{\strut{}0.16}}%
      \csname LTb\endcsname%%
      \put(1473,448){\makebox(0,0){\strut{}1}}%
      \csname LTb\endcsname%%
      \put(2555,448){\makebox(0,0){\strut{}2}}%
      \csname LTb\endcsname%%
      \put(3637,448){\makebox(0,0){\strut{}3}}%
      \csname LTb\endcsname%%
      \put(4718,448){\makebox(0,0){\strut{}4}}%
      \csname LTb\endcsname%%
      \put(5800,448){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}normal/internal frequency}}}%
      \csname LTb\endcsname%%
      \put(6392,2763){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3636,142){\makebox(0,0){\strut{}$ λ $ (homogeneity degree)}}%
      \csname LTb\endcsname%%
      \put(3636,4875){\makebox(0,0){\strut{}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(5800,2766){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=10, η=10$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(5199,2319){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=10, η=8$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(5172,3160){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=8, η=10$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4718,2061){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=8, η=8$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4448,1858){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=10, η=6$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4421,2700){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=6, η=10$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4100,1459){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=8, η=6$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4073,2300){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=6, η=8$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3637,3801){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=6, η=6$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3482,3780){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=10, η=4$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3455,4642){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=4, η=10$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3276,3607){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=8, η=4$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(3249,4468){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=4, η=8$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2987,3279){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=6, η=4$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2960,4120){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=4, η=6$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2555,3003){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=4, η=4$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2194,2806){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=10, η=2$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2167,3665){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=2, η=10$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2122,2861){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=8, η=2$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2095,3702){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=2, η=8$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2014,2766){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=6, η=2$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(1987,3607){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=2, η=6$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(1834,2801){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=4, η=2$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(1806,3642){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=2, η=4$}}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(1473,3012){\rotatebox{-270}{\makebox(0,0){\tiny{$ξ=2, η=2$}}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-nose-freq-rat-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-nose-freq-rat-s-S-xi=10-eta=10-a=1e-1-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(820,651){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(820,1277){\makebox(0,0)[r]{\strut{}0.01}}%
      \csname LTb\endcsname%%
      \put(820,1902){\makebox(0,0)[r]{\strut{}0.02}}%
      \csname LTb\endcsname%%
      \put(820,2527){\makebox(0,0)[r]{\strut{}0.03}}%
      \csname LTb\endcsname%%
      \put(820,3152){\makebox(0,0)[r]{\strut{}0.04}}%
      \csname LTb\endcsname%%
      \put(820,3778){\makebox(0,0)[r]{\strut{}0.05}}%
      \csname LTb\endcsname%%
      \put(820,4403){\makebox(0,0)[r]{\strut{}0.06}}%
      \csname LTb\endcsname%%
      \put(1812,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(2696,448){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(3580,448){\makebox(0,0){\strut{}600}}%
      \csname LTb\endcsname%%
      \put(4465,448){\makebox(0,0){\strut{}800}}%
      \csname LTb\endcsname%%
      \put(5349,448){\makebox(0,0){\strut{}1000}}%
      \csname LTb\endcsname%%
      \put(5567,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5567,1400){\makebox(0,0)[l]{\strut{}0.002}}%
      \csname LTb\endcsname%%
      \put(5567,2148){\makebox(0,0)[l]{\strut{}0.004}}%
      \csname LTb\endcsname%%
      \put(5567,2896){\makebox(0,0)[l]{\strut{}0.006}}%
      \csname LTb\endcsname%%
      \put(5567,3644){\makebox(0,0)[l]{\strut{}0.008}}%
      \csname LTb\endcsname%%
      \put(5567,4391){\makebox(0,0)[l]{\strut{}0.01}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$√a S$ (pink)}}}%
      \csname LTb\endcsname%%
      \put(6341,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$s$ (red)}}}%
      \csname LTb\endcsname%%
      \put(3193,142){\makebox(0,0){\strut{}frequency number}}%
      \csname LTb\endcsname%%
      \put(3193,4875){\makebox(0,0){\strut{}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-nose-freq-rat-s-S-xi=10-eta=10-a=1e-1-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-nose-freq-rat-s-S-xi=10-eta=10-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(932,652){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(932,1593){\makebox(0,0)[r]{\strut{}0.005}}%
      \csname LTb\endcsname%%
      \put(932,2533){\makebox(0,0)[r]{\strut{}0.01}}%
      \csname LTb\endcsname%%
      \put(932,3474){\makebox(0,0)[r]{\strut{}0.015}}%
      \csname LTb\endcsname%%
      \put(932,4414){\makebox(0,0)[r]{\strut{}0.02}}%
      \csname LTb\endcsname%%
      \put(1880,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(2721,448){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(3561,448){\makebox(0,0){\strut{}600}}%
      \csname LTb\endcsname%%
      \put(4402,448){\makebox(0,0){\strut{}800}}%
      \csname LTb\endcsname%%
      \put(5242,448){\makebox(0,0){\strut{}1000}}%
      \csname LTb\endcsname%%
      \put(5455,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5455,1172){\makebox(0,0)[l]{\strut{}0.0001}}%
      \csname LTb\endcsname%%
      \put(5455,1691){\makebox(0,0)[l]{\strut{}0.0002}}%
      \csname LTb\endcsname%%
      \put(5455,2211){\makebox(0,0)[l]{\strut{}0.0003}}%
      \csname LTb\endcsname%%
      \put(5455,2730){\makebox(0,0)[l]{\strut{}0.0004}}%
      \csname LTb\endcsname%%
      \put(5455,3250){\makebox(0,0)[l]{\strut{}0.0005}}%
      \csname LTb\endcsname%%
      \put(5455,3769){\makebox(0,0)[l]{\strut{}0.0006}}%
      \csname LTb\endcsname%%
      \put(5455,4289){\makebox(0,0)[l]{\strut{}0.0007}}%
      \csname LTb\endcsname%%
      \put(5455,4808){\makebox(0,0)[l]{\strut{}0.0008}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$√a S$ (pink)}}}%
      \csname LTb\endcsname%%
      \put(6341,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$s$ (red)}}}%
      \csname LTb\endcsname%%
      \put(3193,142){\makebox(0,0){\strut{}frequency number}}%
      \csname LTb\endcsname%%
      \put(3193,4875){\makebox(0,0){\strut{}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-nose-freq-rat-s-S-xi=10-eta=10-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-nose-freq-rat-s-S-xi=2-eta=2-a=1e-1-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(820,652){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(820,1185){\makebox(0,0)[r]{\strut{}0.01}}%
      \csname LTb\endcsname%%
      \put(820,1718){\makebox(0,0)[r]{\strut{}0.02}}%
      \csname LTb\endcsname%%
      \put(820,2252){\makebox(0,0)[r]{\strut{}0.03}}%
      \csname LTb\endcsname%%
      \put(820,2785){\makebox(0,0)[r]{\strut{}0.04}}%
      \csname LTb\endcsname%%
      \put(820,3318){\makebox(0,0)[r]{\strut{}0.05}}%
      \csname LTb\endcsname%%
      \put(820,3851){\makebox(0,0)[r]{\strut{}0.06}}%
      \csname LTb\endcsname%%
      \put(820,4385){\makebox(0,0)[r]{\strut{}0.07}}%
      \csname LTb\endcsname%%
      \put(1808,448){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(2693,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(3579,448){\makebox(0,0){\strut{}300}}%
      \csname LTb\endcsname%%
      \put(4464,448){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(5349,448){\makebox(0,0){\strut{}500}}%
      \csname LTb\endcsname%%
      \put(5567,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5567,1331){\makebox(0,0)[l]{\strut{}0.002}}%
      \csname LTb\endcsname%%
      \put(5567,2009){\makebox(0,0)[l]{\strut{}0.004}}%
      \csname LTb\endcsname%%
      \put(5567,2688){\makebox(0,0)[l]{\strut{}0.006}}%
      \csname LTb\endcsname%%
      \put(5567,3367){\makebox(0,0)[l]{\strut{}0.008}}%
      \csname LTb\endcsname%%
      \put(5567,4046){\makebox(0,0)[l]{\strut{}0.01}}%
      \csname LTb\endcsname%%
      \put(5567,4724){\makebox(0,0)[l]{\strut{}0.012}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$√a S$ (pink)}}}%
      \csname LTb\endcsname%%
      \put(6341,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$s$ (red)}}}%
      \csname LTb\endcsname%%
      \put(3193,142){\makebox(0,0){\strut{}frequency number}}%
      \csname LTb\endcsname%%
      \put(3193,4875){\makebox(0,0){\strut{}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-nose-freq-rat-s-S-xi=2-eta=2-a=1e-1-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-nose-freq-rat-s-S-xi=2-eta=2-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(932,650){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(932,1529){\makebox(0,0)[r]{\strut{}0.005}}%
      \csname LTb\endcsname%%
      \put(932,2407){\makebox(0,0)[r]{\strut{}0.01}}%
      \csname LTb\endcsname%%
      \put(932,3286){\makebox(0,0)[r]{\strut{}0.015}}%
      \csname LTb\endcsname%%
      \put(932,4164){\makebox(0,0)[r]{\strut{}0.02}}%
      \csname LTb\endcsname%%
      \put(1877,448){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(2718,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(3559,448){\makebox(0,0){\strut{}300}}%
      \csname LTb\endcsname%%
      \put(4401,448){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(5242,448){\makebox(0,0){\strut{}500}}%
      \csname LTb\endcsname%%
      \put(5455,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5455,1354){\makebox(0,0)[l]{\strut{}0.0002}}%
      \csname LTb\endcsname%%
      \put(5455,2057){\makebox(0,0)[l]{\strut{}0.0004}}%
      \csname LTb\endcsname%%
      \put(5455,2759){\makebox(0,0)[l]{\strut{}0.0006}}%
      \csname LTb\endcsname%%
      \put(5455,3462){\makebox(0,0)[l]{\strut{}0.0008}}%
      \csname LTb\endcsname%%
      \put(5455,4164){\makebox(0,0)[l]{\strut{}0.001}}%
      \csname LTb\endcsname%%
      \put(5455,4867){\makebox(0,0)[l]{\strut{}0.0012}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$√a S$ (pink)}}}%
      \csname LTb\endcsname%%
      \put(6341,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$s$ (red)}}}%
      \csname LTb\endcsname%%
      \put(3193,142){\makebox(0,0){\strut{}frequency number}}%
      \csname LTb\endcsname%%
      \put(3193,4875){\makebox(0,0){\strut{}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-nose-freq-rat-s-S-xi=2-eta=2-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-nose-freq-rat-x-p-S-xi=10-eta=10-a=1e-1-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(708,1357){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,2062){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,2767){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,3472){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,4177){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(708,4882){\makebox(0,0)[r]{\strut{}0.6}}%
      \csname LTb\endcsname%%
      \put(1743,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(2671,448){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(3600,448){\makebox(0,0){\strut{}600}}%
      \csname LTb\endcsname%%
      \put(4528,448){\makebox(0,0){\strut{}800}}%
      \csname LTb\endcsname%%
      \put(5456,448){\makebox(0,0){\strut{}1000}}%
      \csname LTb\endcsname%%
      \put(5679,651){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5679,1277){\makebox(0,0)[l]{\strut{}0.01}}%
      \csname LTb\endcsname%%
      \put(5679,1902){\makebox(0,0)[l]{\strut{}0.02}}%
      \csname LTb\endcsname%%
      \put(5679,2527){\makebox(0,0)[l]{\strut{}0.03}}%
      \csname LTb\endcsname%%
      \put(5679,3152){\makebox(0,0)[l]{\strut{}0.04}}%
      \csname LTb\endcsname%%
      \put(5679,3778){\makebox(0,0)[l]{\strut{}0.05}}%
      \csname LTb\endcsname%%
      \put(5679,4403){\makebox(0,0)[l]{\strut{}0.06}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$x$ (blue), $p_x$ (grey)}}}%
      \csname LTb\endcsname%%
      \put(6341,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$√a S$ (pink)}}}%
      \csname LTb\endcsname%%
      \put(3193,142){\makebox(0,0){\strut{}frequency number}}%
      \csname LTb\endcsname%%
      \put(3193,4875){\makebox(0,0){\strut{}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-nose-freq-rat-x-p-S-xi=10-eta=10-a=1e-1-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-nose-freq-rat-x-p-S-xi=10-eta=10-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(708,1345){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,2038){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,2732){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,3425){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,4118){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(708,4811){\makebox(0,0)[r]{\strut{}0.6}}%
      \csname LTb\endcsname%%
      \put(1722,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(2628,448){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(3534,448){\makebox(0,0){\strut{}600}}%
      \csname LTb\endcsname%%
      \put(4440,448){\makebox(0,0){\strut{}800}}%
      \csname LTb\endcsname%%
      \put(5346,448){\makebox(0,0){\strut{}1000}}%
      \csname LTb\endcsname%%
      \put(5567,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5567,1593){\makebox(0,0)[l]{\strut{}0.005}}%
      \csname LTb\endcsname%%
      \put(5567,2533){\makebox(0,0)[l]{\strut{}0.01}}%
      \csname LTb\endcsname%%
      \put(5567,3474){\makebox(0,0)[l]{\strut{}0.015}}%
      \csname LTb\endcsname%%
      \put(5567,4414){\makebox(0,0)[l]{\strut{}0.02}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$x$ (blue), $p_x$ (grey)}}}%
      \csname LTb\endcsname%%
      \put(6341,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$√a S$ (pink)}}}%
      \csname LTb\endcsname%%
      \put(3137,142){\makebox(0,0){\strut{}frequency number}}%
      \csname LTb\endcsname%%
      \put(3137,4875){\makebox(0,0){\strut{}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-nose-freq-rat-x-p-S-xi=10-eta=10-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-nose-freq-rat-x-p-S-xi=2-eta=2-a=1e-1-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(708,1254){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,1855){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,2457){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,3059){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,3660){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(708,4262){\makebox(0,0)[r]{\strut{}0.6}}%
      \csname LTb\endcsname%%
      \put(708,4864){\makebox(0,0)[r]{\strut{}0.7}}%
      \csname LTb\endcsname%%
      \put(1740,448){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(2669,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(3598,448){\makebox(0,0){\strut{}300}}%
      \csname LTb\endcsname%%
      \put(4527,448){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(5456,448){\makebox(0,0){\strut{}500}}%
      \csname LTb\endcsname%%
      \put(5679,652){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5679,1185){\makebox(0,0)[l]{\strut{}0.01}}%
      \csname LTb\endcsname%%
      \put(5679,1718){\makebox(0,0)[l]{\strut{}0.02}}%
      \csname LTb\endcsname%%
      \put(5679,2252){\makebox(0,0)[l]{\strut{}0.03}}%
      \csname LTb\endcsname%%
      \put(5679,2785){\makebox(0,0)[l]{\strut{}0.04}}%
      \csname LTb\endcsname%%
      \put(5679,3318){\makebox(0,0)[l]{\strut{}0.05}}%
      \csname LTb\endcsname%%
      \put(5679,3851){\makebox(0,0)[l]{\strut{}0.06}}%
      \csname LTb\endcsname%%
      \put(5679,4385){\makebox(0,0)[l]{\strut{}0.07}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$x$ (blue), $p_x$ (grey)}}}%
      \csname LTb\endcsname%%
      \put(6341,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$√a S$ (pink)}}}%
      \csname LTb\endcsname%%
      \put(3193,142){\makebox(0,0){\strut{}frequency number}}%
      \csname LTb\endcsname%%
      \put(3193,4875){\makebox(0,0){\strut{}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-nose-freq-rat-x-p-S-xi=2-eta=2-a=1e-1-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> nhnd/nhnd-nose-freq-rat-x-p-S-xi=2-eta=2-mac.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6800.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(708,652){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(708,1255){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(708,1859){\makebox(0,0)[r]{\strut{}0.2}}%
      \csname LTb\endcsname%%
      \put(708,2463){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%%
      \put(708,3066){\makebox(0,0)[r]{\strut{}0.4}}%
      \csname LTb\endcsname%%
      \put(708,3670){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(708,4274){\makebox(0,0)[r]{\strut{}0.6}}%
      \csname LTb\endcsname%%
      \put(708,4877){\makebox(0,0)[r]{\strut{}0.7}}%
      \csname LTb\endcsname%%
      \put(1718,448){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(2625,448){\makebox(0,0){\strut{}200}}%
      \csname LTb\endcsname%%
      \put(3532,448){\makebox(0,0){\strut{}300}}%
      \csname LTb\endcsname%%
      \put(4439,448){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(5346,448){\makebox(0,0){\strut{}500}}%
      \csname LTb\endcsname%%
      \put(5567,650){\makebox(0,0)[l]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5567,1529){\makebox(0,0)[l]{\strut{}0.005}}%
      \csname LTb\endcsname%%
      \put(5567,2407){\makebox(0,0)[l]{\strut{}0.01}}%
      \csname LTb\endcsname%%
      \put(5567,3286){\makebox(0,0)[l]{\strut{}0.015}}%
      \csname LTb\endcsname%%
      \put(5567,4164){\makebox(0,0)[l]{\strut{}0.02}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(186,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$x$ (blue), $p_x$ (grey)}}}%
      \csname LTb\endcsname%%
      \put(6341,2763){\rotatebox{-270}{\makebox(0,0){\strut{}$√a S$ (pink)}}}%
      \csname LTb\endcsname%%
      \put(3137,142){\makebox(0,0){\strut{}frequency number}}%
      \csname LTb\endcsname%%
      \put(3137,4875){\makebox(0,0){\strut{}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={340.00bp},height={255.00bp}]{nhnd/nhnd-nose-freq-rat-x-p-S-xi=2-eta=2-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup

